Prediction Intervals and Confidence Regions for Symbolic Regression Models based on Likelihood Profiles

Symbolic regression is a nonlinear regression method which is commonly performed by an evolutionary computation method such as genetic programming. Quantification of uncertainty of regression models is important for the interpretation of models and for decision making. The linear approximation and so-called likelihood profiles are well-known possibilities for the calculation of confidence and prediction intervals for nonlinear regression models. These simple and effective techniques have been completely ignored so far in the genetic programming literature. In this work we describe the calculation of likelihood profiles in details and also provide some illustrative examples with models created with three different symbolic regression algorithms on two different datasets. The examples highlight the importance of the likelihood profiles to understand the limitations of symbolic regression models and to help the user taking an informed post-prediction decision.

==> figs/Kotanchek_profile.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4220.00,4220.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(310,422){\makebox(0,0)[r]{\strut{}$-2$}}%
      \csname LTb\endcsname%%
      \put(310,844){\makebox(0,0)[r]{\strut{}$-1.5$}}%
      \csname LTb\endcsname%%
      \put(310,1266){\makebox(0,0)[r]{\strut{}$-1$}}%
      \csname LTb\endcsname%%
      \put(310,1688){\makebox(0,0)[r]{\strut{}$-0.5$}}%
      \csname LTb\endcsname%%
      \put(310,2110){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(310,2531){\makebox(0,0)[r]{\strut{}$0.5$}}%
      \csname LTb\endcsname%%
      \put(310,2953){\makebox(0,0)[r]{\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(310,3375){\makebox(0,0)[r]{\strut{}$1.5$}}%
      \csname LTb\endcsname%%
      \put(310,3797){\makebox(0,0)[r]{\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(422,218){\makebox(0,0){\strut{}$1.86$}}%
      \csname LTb\endcsname%%
      \put(486,218){\makebox(0,0){\strut{}$1.88$}}%
      \csname LTb\endcsname%%
      \put(549,218){\makebox(0,0){\strut{}$1.9$}}%
      \csname LTb\endcsname%%
      \put(613,218){\makebox(0,0){\strut{}$1.92$}}%
      \csname LTb\endcsname%%
      \put(676,218){\makebox(0,0){\strut{}$1.94$}}%
      \csname LTb\endcsname%%
      \put(740,218){\makebox(0,0){\strut{}$1.96$}}%
      \csname LTb\endcsname%%
      \put(803,218){\makebox(0,0){\strut{}$1.98$}}%
      \csname LTb\endcsname%%
      \put(867,218){\makebox(0,0){\strut{}$2$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(910,218){\makebox(0,0){\strut{}$1.93$}}%
      \csname LTb\endcsname%%
      \put(955,218){\makebox(0,0){\strut{}$1.94$}}%
      \csname LTb\endcsname%%
      \put(999,218){\makebox(0,0){\strut{}$1.95$}}%
      \csname LTb\endcsname%%
      \put(1044,218){\makebox(0,0){\strut{}$1.96$}}%
      \csname LTb\endcsname%%
      \put(1088,218){\makebox(0,0){\strut{}$1.97$}}%
      \csname LTb\endcsname%%
      \put(1133,218){\makebox(0,0){\strut{}$1.98$}}%
      \csname LTb\endcsname%%
      \put(1178,218){\makebox(0,0){\strut{}$1.99$}}%
      \csname LTb\endcsname%%
      \put(1222,218){\makebox(0,0){\strut{}$2$}}%
      \csname LTb\endcsname%%
      \put(1267,218){\makebox(0,0){\strut{}$2.01$}}%
      \csname LTb\endcsname%%
      \put(1311,218){\makebox(0,0){\strut{}$2.02$}}%
      \csname LTb\endcsname%%
      \put(1356,218){\makebox(0,0){\strut{}$2.03$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1398,218){\makebox(0,0){\strut{}$0.042$}}%
      \csname LTb\endcsname%%
      \put(1472,218){\makebox(0,0){\strut{}$0.044$}}%
      \csname LTb\endcsname%%
      \put(1547,218){\makebox(0,0){\strut{}$0.046$}}%
      \csname LTb\endcsname%%
      \put(1621,218){\makebox(0,0){\strut{}$0.048$}}%
      \csname LTb\endcsname%%
      \put(1695,218){\makebox(0,0){\strut{}$0.05$}}%
      \csname LTb\endcsname%%
      \put(1770,218){\makebox(0,0){\strut{}$0.052$}}%
      \csname LTb\endcsname%%
      \put(1844,218){\makebox(0,0){\strut{}$0.054$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(1886,218){\makebox(0,0){\strut{}$0.975$}}%
      \csname LTb\endcsname%%
      \put(1942,218){\makebox(0,0){\strut{}$0.98$}}%
      \csname LTb\endcsname%%
      \put(1997,218){\makebox(0,0){\strut{}$0.985$}}%
      \csname LTb\endcsname%%
      \put(2053,218){\makebox(0,0){\strut{}$0.99$}}%
      \csname LTb\endcsname%%
      \put(2109,218){\makebox(0,0){\strut{}$0.995$}}%
      \csname LTb\endcsname%%
      \put(2165,218){\makebox(0,0){\strut{}$1$}}%
      \csname LTb\endcsname%%
      \put(2220,218){\makebox(0,0){\strut{}$1.005$}}%
      \csname LTb\endcsname%%
      \put(2276,218){\makebox(0,0){\strut{}$1.01$}}%
      \csname LTb\endcsname%%
      \put(2332,218){\makebox(0,0){\strut{}$1.015$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2375,218){\makebox(0,0){\strut{}$-0.0094$}}%
      \csname LTb\endcsname%%
      \put(2431,218){\makebox(0,0){\strut{}$-0.0092$}}%
      \csname LTb\endcsname%%
      \put(2486,218){\makebox(0,0){\strut{}$-0.009$}}%
      \csname LTb\endcsname%%
      \put(2542,218){\makebox(0,0){\strut{}$-0.0088$}}%
      \csname LTb\endcsname%%
      \put(2598,218){\makebox(0,0){\strut{}$-0.0086$}}%
      \csname LTb\endcsname%%
      \put(2653,218){\makebox(0,0){\strut{}$-0.0084$}}%
      \csname LTb\endcsname%%
      \put(2709,218){\makebox(0,0){\strut{}$-0.0082$}}%
      \csname LTb\endcsname%%
      \put(2764,218){\makebox(0,0){\strut{}$-0.008$}}%
      \csname LTb\endcsname%%
      \put(2820,218){\makebox(0,0){\strut{}$-0.0078$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(2863,218){\makebox(0,0){\strut{}0.00017}}%
      \csname LTb\endcsname%%
      \put(2927,218){\makebox(0,0){\strut{}0.00017}}%
      \csname LTb\endcsname%%
      \put(2990,218){\makebox(0,0){\strut{}0.00018}}%
      \csname LTb\endcsname%%
      \put(3054,218){\makebox(0,0){\strut{}0.00018}}%
      \csname LTb\endcsname%%
      \put(3117,218){\makebox(0,0){\strut{}0.00019}}%
      \csname LTb\endcsname%%
      \put(3181,218){\makebox(0,0){\strut{}0.00019}}%
      \csname LTb\endcsname%%
      \put(3244,218){\makebox(0,0){\strut{}0.00020}}%
      \csname LTb\endcsname%%
      \put(3308,218){\makebox(0,0){\strut{}0.00020}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(3351,218){\makebox(0,0){\strut{}$0.0215$}}%
      \csname LTb\endcsname%%
      \put(3401,218){\makebox(0,0){\strut{}$0.022$}}%
      \csname LTb\endcsname%%
      \put(3450,218){\makebox(0,0){\strut{}$0.0225$}}%
      \csname LTb\endcsname%%
      \put(3500,218){\makebox(0,0){\strut{}$0.023$}}%
      \csname LTb\endcsname%%
      \put(3549,218){\makebox(0,0){\strut{}$0.0235$}}%
      \csname LTb\endcsname%%
      \put(3599,218){\makebox(0,0){\strut{}$0.024$}}%
      \csname LTb\endcsname%%
      \put(3648,218){\makebox(0,0){\strut{}$0.0245$}}%
      \csname LTb\endcsname%%
      \put(3698,218){\makebox(0,0){\strut{}$0.025$}}%
      \csname LTb\endcsname%%
      \put(3747,218){\makebox(0,0){\strut{}$0.0255$}}%
      \csname LTb\endcsname%%
      \put(3797,218){\makebox(0,0){\strut{}$0.026$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Kotanchek_profile_pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup


==> figs/TIR-Kotanchek_profile.tex <==
% GNUPLOT: LaTeX picture with Postscript
\begingroup
  \makeatletter
  \providecommand\color[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package color not loaded in conjunction with
      terminal option `colourtext'%
    }{See the gnuplot documentation for explanation.%
    }{Either use 'blacktext' in gnuplot or load the package
      color.sty in LaTeX.}%
    \renewcommand\color[2][]{}%
  }%
  \providecommand\includegraphics[2][]{%
    \GenericError{(gnuplot) \space\space\space\@spaces}{%
      Package graphicx or graphics not loaded%
    }{See the gnuplot documentation for explanation.%
    }{The gnuplot epslatex terminal needs graphicx.sty or graphics.sty.}%
    \renewcommand\includegraphics[2][]{}%
  }%
  \providecommand\rotatebox[2]{#2}%
  \@ifundefined{ifGPcolor}{%
    \newif\ifGPcolor
    \GPcolortrue
  }{}%
  \@ifundefined{ifGPblacktext}{%
    \newif\ifGPblacktext
    \GPblacktexttrue
  }{}%
  % define a \g@addto@macro without @ in the name:
  \let\gplgaddtomacro\g@addto@macro
  % define empty templates for all commands taking text:
  \gdef\gplbacktext{}%
  \gdef\gplfronttext{}%
  \makeatother
  \ifGPblacktext
    % no textcolor at all
    \def\colorrgb#1{}%
    \def\colorgray#1{}%
  \else
    % gray or color?
    \ifGPcolor
      \def\colorrgb#1{\color[rgb]{#1}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color[rgb]{1,0,0}}%
      \expandafter\def\csname LT1\endcsname{\color[rgb]{0,1,0}}%
      \expandafter\def\csname LT2\endcsname{\color[rgb]{0,0,1}}%
      \expandafter\def\csname LT3\endcsname{\color[rgb]{1,0,1}}%
      \expandafter\def\csname LT4\endcsname{\color[rgb]{0,1,1}}%
      \expandafter\def\csname LT5\endcsname{\color[rgb]{1,1,0}}%
      \expandafter\def\csname LT6\endcsname{\color[rgb]{0,0,0}}%
      \expandafter\def\csname LT7\endcsname{\color[rgb]{1,0.3,0}}%
      \expandafter\def\csname LT8\endcsname{\color[rgb]{0.5,0.5,0.5}}%
    \else
      % gray
      \def\colorrgb#1{\color{black}}%
      \def\colorgray#1{\color[gray]{#1}}%
      \expandafter\def\csname LTw\endcsname{\color{white}}%
      \expandafter\def\csname LTb\endcsname{\color{black}}%
      \expandafter\def\csname LTa\endcsname{\color{black}}%
      \expandafter\def\csname LT0\endcsname{\color{black}}%
      \expandafter\def\csname LT1\endcsname{\color{black}}%
      \expandafter\def\csname LT2\endcsname{\color{black}}%
      \expandafter\def\csname LT3\endcsname{\color{black}}%
      \expandafter\def\csname LT4\endcsname{\color{black}}%
      \expandafter\def\csname LT5\endcsname{\color{black}}%
      \expandafter\def\csname LT6\endcsname{\color{black}}%
      \expandafter\def\csname LT7\endcsname{\color{black}}%
      \expandafter\def\csname LT8\endcsname{\color{black}}%
    \fi
  \fi
    \setlength{\unitlength}{0.0500bp}%
    \ifx\gptboxheight\undefined%
      \newlength{\gptboxheight}%
      \newlength{\gptboxwidth}%
      \newsavebox{\gptboxtext}%
    \fi%
    \setlength{\fboxrule}{0.5pt}%
    \setlength{\fboxsep}{1pt}%
\begin{picture}(4220.00,1680.00)%
    \gplgaddtomacro\gplbacktext{%
      \csname LTb\endcsname%%
      \put(521,595){\makebox(0,0)[r]{\strut{}$-1$}}%
      \csname LTb\endcsname%%
      \put(521,928){\makebox(0,0)[r]{\strut{}$0$}}%
      \csname LTb\endcsname%%
      \put(521,1261){\makebox(0,0)[r]{\strut{}$1$}}%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(111,923){\rotatebox{-270}{\makebox(0,0){\strut{}$\Tau$}}}%
      \csname LTb\endcsname%%
      \put(879,132){\makebox(0,0){\strut{}$\theta_{0}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1413,132){\makebox(0,0){\strut{}$\theta_{1}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(1947,132){\makebox(0,0){\strut{}$\theta_{2}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(2482,132){\makebox(0,0){\strut{}$\theta_{3}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3016,132){\makebox(0,0){\strut{}$\theta_{4}$}}%
    }%
    \gplgaddtomacro\gplbacktext{%
    }%
    \gplgaddtomacro\gplfronttext{%
      \csname LTb\endcsname%%
      \put(3551,132){\makebox(0,0){\strut{}$\theta_{5}$}}%
    }%
    \gplbacktext
    \put(0,0){\includegraphics{Kotanchek_profile_pdf}}%
    \gplfronttext
  \end{picture}%
\endgroup

